Learning Fitness Functions for Machine Programming

The problem of automatic software generation is known as Machine Programming. In this work, we propose a framework based on genetic algorithms to solve this problem. Although genetic algorithms have been used successfully for many problems, one criticism is that hand-crafting its fitness function, the test that aims to effectively guide its evolution, can be notably challenging. Our framework presents a novel approach to learn the fitness function using neural networks to predict values of ideal fitness functions. We also augment the evolutionary process with a minimally intrusive search heuristic. This heuristic improves the framework's ability to discover correct programs from ones that are approximately correct and does so with negligible computational overhead. We compare our approach with several state-of-the-art program synthesis methods and demonstrate that it finds more correct programs with fewer candidate program generations.

==> TODO.tex <==
\begin{TODO}
\begin{itemize}
    \item Compare results with original Deepcoder or any other state of the art program synthesis tools.
    
    \item Increase the program length to see how does our framework generalize.
    
    \item Use time to compare results.
    
    \item Add more references of genetic algorithm works. 
    
\end{itemize}
\end{TODO}

==> app-loss-figure.tex <==
\begin{figure}[htpb]
    \centering
    
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=1\linewidth]{./FIGS/NEWMODEL/model_cat_confusion_matrix_CF}
    \vspace{-0.2cm}
    \caption{$\scheme_{CF}$}
    \end{subfigure}
    %\quad
    %~
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=1\linewidth]{./FIGS/NEWMODEL/model_cat_confusion_matrix_LCS}
     \vspace{-0.2cm}
     \caption{$\scheme_{LCS}$}
    \end{subfigure}
    %~
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=1\linewidth]{./FIGS/NEWMODEL/FP_acc}
     \vspace{-0.2cm}
     \caption{$\scheme_{FP}$}
    \end{subfigure}
    %\\
    \caption{Confusion matrix of (a) $\scheme_{CF}$ (b) $\scheme_{LCS}$ score and (c) $\scheme_{FP}$ accuracy over epochs on validation data.}
    \label{fig_total_found}
    \vspace{-0.2cm}
\end{figure}

==> app-oldtable.tex <==
\begin{table*}[t]
  %\scriptsize
  %\parbox{0.3\linewidth}{
 % \begin{minipage}{\columnwidth}
    \caption{Comparison with DeepCoder and PCCoder in synthesizing different length programs. All experiments are done with the maximum search space set to 3,000,000 candidate programs.}
  %\vspace{0.5cm}
  \label{table:compare}
  %\scalebox{0.9}{
  \vskip 0.15in
  \begin{center}
  \begin{small}
  \begin{sc}
  \begin{tabular}{clccccccccccc}
  \hline\hline
  Program & \multirow{2}{*}{Method} & Synthesis & \multicolumn{10}{c}{Time Required to Synthesize (in seconds)} \\\cline{4-13}
  Length & & Percentage & 10\% & 20\% & 30\% & 40\% & 50\% & 60\% & 70\% & 80\% & 90\% & 100\%\\\hline\hline 
  
  \multirow{5}{*}{5}
  & $\mathit{Constant}$ & 48\% & $<$1s & 60s & 388s & 422s & - & - & - & - & - &- \\
  & $\mathit{Edit}$ & 77\% & $<$1s & 7s & 112s & 272s & 345s & 393s & 483s & - & - &- \\
  & $\mathit{DeepCoder}$ & 40\% & $<$1s & $<$1s & 2s & 126s & - & - & - & - & - &- \\
  & $\mathit{PCCoder}$ & 51\% & 1s & 1s & 6s & 66s & 357s & - & - & - & - & - \\ 
  & $\mathit{\scheme_{FP}}$ & 64\% & $<$1s & $<$1s & 4s & 174s & 525s & 803s & - & - & - & - \\  
  %& $\mathit{\scheme_{FP}-Opt}$ & 64\% & $<$1s & $<$1s & 1s & 164s & 515s & 793s & - & - & - & - \\
  & $\mathit{\scheme_{LCS}}$ & 98\% & $<$1s & $<$1s & 4s & 43s & 112s & 349s & 600s & 690s & 838s & - \\
  %& $\mathit{\scheme_{LCS}-Opt}$ & 98\% & $<$1s & $<$1s & 1s & 11s & 33s & 141s & 321s & 421s & 537s & - \\
  & $\mathit{\scheme_{CF}}$ &  96\% & $<$1s & $<$1s & 3s & 46s & 131s & 392s & 671s & 768s & 874s & - \\
  %& $\mathit{\scheme_{CF}-Opt}$ &  96\% & $<$1s & $<$1s & 1s & 13s & 39s & 181s & 380s & 475s & 569s & - \\
  & $\mathit{\scheme_{LCS+Local search}}$ &  98\% & $<$1s & $<$1s & 4s & 43s & 115s & 344s & 612s & 704s & 847s & - \\
  & $\mathit{\scheme_{CF+Local search}}$ &  96\% & $<$1s & $<$1s & 3s & 47s & 138s & 400s & 660s & 753s & 866s & - \\
  & $\mathit{Oracle_{LCS|CF}}$ & 100\% & $<$1s & $<$1s & $<$1s & $<$1s & $<$1s & $<$1s & 1s & 1s & 1s & 1s \\
  \hline\hline 
  
  \multirow{5}{*}{6} 
  & $\mathit{Constant}$ & 43\% & $<$1s & 1s & 314s & 397s & - & - & - & - & - &- \\
  & $\mathit{Edit}$ & 73\% & $<$1s & 1s & 82s & 229s & 300s & 368s & 462s & - & - &- \\
  & $\mathit{DeepCoder}$ & 45\% & $<$1s & $<$1s & $<$1s & 14s & - & - & - & - & - &- \\
  & $\mathit{PCCoder}$ & 75\% & 1s & 1s & 1s & 4s & 190s & 233s & 619s & - & - & - \\ 
  & $\mathit{\scheme_{FP}}$ & 63\% & $<$1s & $<$1s & 3s & 306s & 464s & 919s & - & - & - & - \\  
  %& $\mathit{\scheme_{FP}-Opt}$ & 63\% & $<$1s & $<$1s & 1s & 296s & 457s & 909s & - & - & - & - \\
  & $\mathit{\scheme_{LCS}}$ & 87\% & $<$1s & $<$1s & 4s & 130s & 574s & 716s & 870s & 956s & - & - \\
  %& $\mathit{\scheme_{LCS}-Opt}$ & 87\% & $<$1s & $<$1s & 1s & 56s & 307s & 429s & 579s & 658s & - & - \\
  & $\mathit{\scheme_{CF}}$ &  88\% & $<$1s & $<$1s & 3s & 183s & 533s & 732s & 872s & 918s & - & - \\
  %& $\mathit{\scheme_{CF}-Opt}$ & 88\% & $<$1s & $<$1s & 1s & 66s & 281s & 435s & 569s & 612s & - & - \\
  & $\mathit{\scheme_{LCS+Local search}}$ &  87\% & $<$1s & $<$1s & 4s & 127s & 563s & 695s & 875s & 937s & - & - \\
  & $\mathit{\scheme_{CF+Local search}}$ &  88\% & $<$1s & $<$1s & 3s & 185s & 528s & 754s & 855s & 899s & - & - \\
  & $\mathit{Oracle_{LCS|CF}}$ & 100\% & $<$1s & $<$1s & $<$1s & $<$1s & $<$1s & $<$1s & 1s & 1s & 1s & 1s \\
  \hline\hline 
  
  \multirow{5}{*}{7} 
  & $\mathit{Constant}$ & 44\% & $<$1s & 1s & 1s & 685s & - & - & - & - & - &- \\
  & $\mathit{Edit}$ & 68\% & $<$1s & 1s & 1s & 249s & 354s & 433s & - & - & - &- \\
  & $\mathit{DeepCoder}$ & 45\% & $<$1s & $<$1s & $<$1s & 13s & - & - & - & - & - &- \\
  & $\mathit{PCCoder}$ & 52\% & 1s & 1s & 2s & 11s & 635s & - & - & - & - & - \\ 
  & $\mathit{\scheme_{FP}}$ & 58\% & $<$1s & $<$1s & $<$1s & 393s & 566s & - & - & - & - & - \\  
  %& $\mathit{\scheme_{FP}-Opt}$ & 58\% & $<$1s & $<$1s & $<$1s & 383s & 556s & - & - & - & - & - \\
  & $\mathit{\scheme_{LCS}}$ & 81\% & $<$1s & $<$1s & $<$1s & 176s & 676s & 1062s & 1134s & 1180s & - & - \\
  %& $\mathit{\scheme_{LCS}-Opt}$ & 81\% & $<$1s & $<$1s & $<$1s & 92s & 445s & 775s & 834s & 886s & - & - \\
  & $\mathit{\scheme_{CF}}$ &  78\% & $<$1s & $<$1s & $<$1s & 127s & 609s & 889s & 956s & - & - & - \\
  %& $\mathit{\scheme_{CF}-Opt}$ & 78\% & $<$1s & $<$1s & $<$1s & 49s & 349s & 593s & 655s & - & - & - \\
  & $\mathit{\scheme_{LCS+Local search}}$ &  81\% & $<$1s & $<$1s & $<$1s & 178s & 670s & 1094s & 1112s & 1156s & - & - \\
  & $\mathit{\scheme_{CF+Local search}}$ &  79\% & $<$1s & $<$1s & $<$1s & 126s & 624s & 876s & 976s & - & - & - \\
  & $\mathit{Oracle_{LCS|CF}}$ & 100\% & $<$1s & $<$1s & $<$1s & $<$1s & $<$1s & $<$1s & 1s & 1s & 1s & 1s \\
  \hline\hline

  \multirow{5}{*}{8} 
  & $\mathit{Constant}$ & 43\% & $<$1s & 1s & 1s & 1371s & - & - & - & - & - &- \\
  & $\mathit{Edit}$ & 65\% & $<$1s & 1s & 1s & 297s & 401s & 534s & - & - & - &- \\
  & $\mathit{DeepCoder}$ & 56\% & $<$1s & $<$1s & $<$1s & $<$1s & 29s & - & - & - & - &- \\
  & $\mathit{PCCoder}$ & 57\% & 1s & 1s & 1s & 1s & 15s & - & - & - & - & - \\ 
  & $\mathit{\scheme_{FP}}$ & 49\% & $<$1s & $<$1s & $<$1s & 587s & - & - & - & - & - & - \\  
  %& $\mathit{\scheme_{FP}-Opt}$ & 49\% & $<$1s & $<$1s & $<$1s & 577s & - & - & - & - & - & - \\
  & $\mathit{\scheme_{LCS}}$ & 68\% & $<$1s & $<$1s & $<$1s & 748s & 1545s & 1702s & - & - & - & - \\
  %& $\mathit{\scheme_{LCS}-Opt}$ & 68\% & $<$1s & $<$1s & $<$1s & 571s & 1258s & 1401s & - & - & - & - \\
  & $\mathit{\scheme_{CF}}$ &  69\% & $<$1s & $<$1s & $<$1s & 404s & 988s & 1044s & - & - & - & - \\
  %& $\mathit{\scheme_{CF}-Opt}$ & 69\% & $<$1s & $<$1s & $<$1s & 236s & 699s & 745s & - & - & - & - \\
  & $\mathit{\scheme_{LCS+Local search}}$ &  68\% & $<$1s & $<$1s & $<$1s & 763s & 1578s & 1668s & - & - & - & - \\
  & $\mathit{\scheme_{CF+Local search}}$ &  69\% & $<$1s & $<$1s & $<$1s & 392s & 969s & 1013s & - & - & - & - \\
  & $\mathit{Oracle_{LCS|CF}}$ & 100\% & $<$1s & $<$1s & $<$1s & $<$1s & $<$1s & $<$1s & 1s & 1s & 1s & 1s \\
  \hline\hline
  
  \multirow{5}{*}{9} 
  % this section will be updated. 
  & $\mathit{Constant}$ & 41\% & $<$1s & 1s & 1s & 1387s & - & - & - & - & - &- \\
  & $\mathit{Edit}$ & 67\% & $<$1s & 1s & 1s & 288s & 429s & 574s & - & - & - &- \\
  & $\mathit{DeepCoder}$ & 53\% & $<$1s & $<$1s & $<$1s & $<$1s & 56s & - & - & - & - & -\\
  & $\mathit{PCCoder}$ & 55\% & 1s & 1s & 1s & 1s & 107s & - & - & - & - & - \\ 
  & $\mathit{\scheme_{FP}}$ & 52\% & $<$1s & $<$1s & $<$1s & $<$1s & 614s & - & - & - & - & - \\  
  %& $\mathit{\scheme_{FP}-Opt}$ & 59\% & $<$1s & $<$1s & $<$1s & $<$1s & 605s & - & - & - & - & - \\
  & $\mathit{\scheme_{LCS}}$ & 64\% & $<$1s & $<$1s & $<$1s &  1584s & 2544s & 2846s & - & - & - & - \\
  %& $\mathit{\scheme_{LCS}-Opt}$ & 73\% & $<$1s & $<$1s & $<$1s & $<$1s & 1808s & 2667s & 3644s & - & - & - \\
  & $\mathit{\scheme_{CF}}$ &  67\% & $<$1s & $<$1s & $<$1s & 837s & 1055s & 1195s & - & - & - & - \\
  %& $\mathit{\scheme_{CF}-Opt}$ & 76\% & $<$1s & $<$1s & $<$1s & $<$1s & 489s & 744s & 798s & - & - & - \\
  & $\mathit{\scheme_{LCS+Local search}}$ &  64\% & $<$1s & $<$1s & 1s &  1603s & 2473s & 2790s & - & - & - & - \\
  & $\mathit{\scheme_{CF+Local search}}$ &  67\% & $<$1s & $<$1s & 1s & 846s & 1029s & 1207s & - & - & - & - \\
  & $\mathit{Oracle_{LCS|CF}}$ & 100\% & $<$1s & $<$1s & $<$1s & $<$1s & $<$1s & $<$1s & 1s & 1s & 1s & 1s \\
  \hline\hline
  
  
  \multirow{5}{*}{10}
  & $\mathit{Constant}$ & 41\% & $<$1s & 1s & 1s & 1403s & - & - & - & - & - &- \\
  & $\mathit{Edit}$ & 68\% & $<$1s & 1s & 1s & 208s & 459s & 591s & - & - & - &- \\
  & $\mathit{DeepCoder}$ & 42\% & $<$1s & $<$1s & $<$1s & 67s & - & - & - & - & - & -\\
  & $\mathit{PCCoder}$ & 48\% & 1s & 1s & 1s & 1011s & - & - & - & - & - & - \\ 
  & $\mathit{\scheme_{FP}}$ & 49\% & $<$1s & $<$1s & $<$1s & 517s & - & - & - & - & - & - \\  
  %& $\mathit{\scheme_{FP}-Opt}$ & 49\% & $<$1s & $<$1s & $<$1s & 507s & - & - & - & - & - & - \\
  & $\mathit{\scheme_{LCS}}$ & 55\% & $<$1s & $<$1s & $<$1s & 625s & 1640s & - & - & - & - & - \\
  %& $\mathit{\scheme_{LCS}-Opt}$ & 55\% & $<$1s & $<$1s & $<$1s & 595s & 1523s & - & - & - & - & - \\
  & $\mathit{\scheme_{CF}}$ & 66\% & $<$1s & $<$1s & $<$1s & 164s & 957s & 1121s & - & - & - & - \\
  %& $\mathit{\scheme_{CF}-Opt}$ & 66\% & $<$1s & $<$1s & $<$1s & 85s & 674s & 826s & - & - & - & - \\
  & $\mathit{\scheme_{LCS+Local search}}$ &  55\% & $<$1s & $<$1s & $<$1s & 638s & 1649s & - & - & - & - & - \\
  & $\mathit{\scheme_{CF+Local search}}$ &  66\% & $<$1s & $<$1s & $<$1s & 168s & 978s & 1099s & - & - & - & - \\
  & $\mathit{Oracle_{LCS|CF}}$ & 100\% & $<$1s & $<$1s & $<$1s & $<$1s & $<$1s & $<$1s & 1s & 1s & 1s & 1s \\
  \hline\hline
  
  \end{tabular}%}
  %}
% \end{minipage}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

Figure~\ref{table:compare} shows detailed numerical results using synthesis time as the metric. Columns 10\% to 100\% show the duration of time (in seconds) it takes to synthesize the corresponding percentage of programs. 

\begin{table*}[t]
\caption{Comparison with DeepCoder and PCCoder in terms of search space use. All experiments are done with the maximum search space set to 3,000,000 candidate programs.}
  \label{table:compare2}
  \begin{center}
\begin{small}
\begin{sc}
  %\scriptsize
  %\parbox{0.3\linewidth}{
 % \begin{minipage}{\columnwidth}
%   \scalebox{0.9}{
  \begin{tabular}{clcccccccccc}
  \hline\hline
  Program & \multirow{2}{*}{Method} & \multicolumn{10}{c}{Search Space Used to Synthesize} \\\cline{3-12}
  Length & & 10\% & 20\% & 30\% & 40\% & 50\% & 60\% & 70\% & 80\% & 90\% & 100\% \\
  \hline\hline 
  
  \multirow{5}{*}{5} 
  & $\mathit{Constant}$ & $<$1\% &	9\% &	59\% &	64\% &	- &	- &	- &	- &	- &	-\\
  & $\mathit{Edit}$ & $<$1\% &	1\% &	17\% &	41\% &	52\% &	60\% &	73\% &	- &	- &	-\\
  & $\mathit{DeepCoder}$ & $<$1\% &	1\% &	1\% &	37\% &	- &	- &	- &	- &	- &	-\\
  & $\mathit{PCCoder}$ & $<$1\% &	1\% &	1\% &	7\% &	33\% &	- &	- &	- &	- &	-\\ 
  & $\mathit{\scheme_{FP}}$ & $<$1\% &  $<$1\% &	1\% &  2\% &	5\% &	23\% &	- &	- &	- &	- \\
  & $\mathit{\scheme_{LCS}}$ & $<$1\% &	1\% &	1\% &	3\% &	7\% &	10\% &	15\% &	21\% &	30\% &	-\\
  & $\mathit{\scheme_{CF}}$ & $<$1\% & 1\% & 1\% &	2\% &	5\% &	9\% &	14\% &	21\% &	29\% & 	- \\
  & $\mathit{\scheme_{LCS+Local search}}$ & $<$1\% &	1\% &	1\% &	2\% &	7\% &	9\% &	15\% &	21\% &	30\% &	-\\
  & $\mathit{\scheme_{CF+Local search}}$ & $<$1\% & 1\% & 1\% &	2\% &	5\% &	9\% &	13\% &	20\% &	28\% & 	- \\
  & $\mathit{Oracle_{LCS|CF}}$ & $<$1\% &	$<$1\% &	$<$1\% &	$<$1\% &	$<$1\% &	$<$1\% &	$<$1\% & $<$1\% & $<$1\% & $<$1\% \\
  \hline\hline 
  
  \multirow{5}{*}{6} 


  & $\mathit{Constant}$ & $<$1\% &	1\% &	46\% &	58\%  &	- &	- &	- &	- &	- &	-\\
  & $\mathit{Edit}$ & $<$1\% &	1\% &	12\% & 33\%  &	43\% &	53\% &	67\% &	- &	- &	-\\
  & $\mathit{DeepCoder}$ & $<$1\% &	1\% &	1\% &	4\%  &	- &	- &	- &	- &	- &	-\\
  & $\mathit{PCCoder}$ & $<$1\% &	$<$1\% &	1\% &	1\% &	33\% &	55\% &	73\% &	- &	- &	-\\ 
  & $\mathit{\scheme_{FP}}$ & $<$1\% &	$<$1\% & 	$<$1\% &	1\% &	5\% &	28\%  &	- &	- &	- &	- \\
  & $\mathit{\scheme_{LCS}}$ & $<$1\% &	$<$1\% &	1\% &	2\% &	5\% &	12\% &	18\% &	25\% &	- &	-\\
  & $\mathit{\scheme_{CF}}$ & $<$1\% &	$<$1\% &	1\% &	2\% &	5\% &	10\% &	17\% &	24\%  &	- & 	- \\
  & $\mathit{\scheme_{LCS+Local search}}$ & $<$1\% &	$<$1\% &	1\% &	1\% &	4\% &	11\% &	18\% &	24\% &	- &	-\\
  & $\mathit{\scheme_{CF+Local search}}$ & $<$1\% &	$<$1\% &	1\% &	2\% &	4\% &	10\% &	16\% &	23\%  &	- & 	- \\
  & $\mathit{Oracle_{LCS|CF}}$ & $<$1\% &	$<$1\% &	$<$1\% &	$<$1\% &	$<$1\% &	$<$1\% &	$<$1\% & $<$1\% & $<$1\% & $<$1\% \\
  \hline\hline 

  \multirow{5}{*}{7} 

  
  & $\mathit{Constant}$ & $<$1\% &	1\% &	1\% &	82\%  &	- &	- &	- &	- &	- &	-\\
  & $\mathit{Edit}$ & $<$1\% &	1\% &	1\% &	34\%  &	48\% &	59\% &	- &	- &	- &	-\\
  & $\mathit{DeepCoder}$ & $<$1\% &	$<$1\% &	1\% &	3\%  &	- &	- &	- &	- &	- &	-\\
  & $\mathit{PCCoder}$ & $<$1\% &	$<$1\% &	1\% &	1\% &	38\% &	- &	- &	- &	- &	-\\ 
  & $\mathit{\scheme_{FP}}$ & $<$1\% &	$<$1\% & 	$<$1\% &	1\% &	14\% &	-  &	- &	- &	- &	- \\
  & $\mathit{\scheme_{LCS}}$ & $<$1\% &	$<$1\% &	$<$1\% &	2\% &	3\% &	6\% &	18\% &	30\% &	- &	-\\
  & $\mathit{\scheme_{CF}}$ & $<$1\% &	$<$1\% &	$<$1\% &	2\% &	5\% &	11\% &	20\% &	-  &	- & 	- \\
  & $\mathit{\scheme_{LCS+Local search}}$ & $<$1\% &	$<$1\% &	$<$1\% &	2\% &	2\% &	6\% &	17\% &	29\% &	- &	-\\
  & $\mathit{\scheme_{CF+Local search}}$ & $<$1\% &	$<$1\% &	$<$1\% &	1\% &	5\% &	10\% &	20\% &	-  &	- & 	- \\
  & $\mathit{Oracle_{LCS|CF}}$ & $<$1\% &	$<$1\% &	$<$1\% &	$<$1\% &	$<$1\% &	$<$1\% &	$<$1\% & $<$1\% & $<$1\% & $<$1\% \\
  \hline\hline   

  \multirow{5}{*}{8} 
  & $\mathit{Constant}$ & $<$1\% &	1\% &	1\% &	93\%  &	- &	- &	- &	- &	- &	-\\
  & $\mathit{Edit}$ & $<$1\% &	1\% &	1\% &	37\%  &	50\% &	67\% &	- &	- &	- &	-\\
  & $\mathit{DeepCoder}$ & $<$1\% &	$<$1\% &	$<$1\% &	1\%  &	6\% &	- &	- &	- &	- &	-\\
  & $\mathit{PCCoder}$ & $<$1\% &	$<$1\% &	$<$1\% &	1\% &	1\% &	- &	- &	- &	- &	-\\ 
  & $\mathit{\scheme_{FP}}$ & $<$1\% &	$<$1\% & 	$<$1\% &	1\% &	- &	-  &	- &	- &	- &	- \\
  & $\mathit{\scheme_{LCS}}$ & $<$1\% &	$<$1\% &	$<$1\% &	3\% &	7\% &	17\% &	- &	- &	- &	-\\
  & $\mathit{\scheme_{CF}}$ & $<$1\% &	$<$1\% &	$<$1\% &	2\% &	6\% &	13\% &	- &	-  & - & 	- \\
  & $\mathit{\scheme_{LCS+Local search}}$ & $<$1\% &	$<$1\% &	$<$1\% &	3\% &	7\% &	16\% &	- &	- &	- &	-\\
  & $\mathit{\scheme_{CF+Local search}}$ & $<$1\% &	$<$1\% &	$<$1\% &	2\% &	5\% &	12\% &	- &	-  & - & 	- \\
  & $\mathit{Oracle_{LCS|CF}}$ & $<$1\% &	$<$1\% &	$<$1\% &	$<$1\% &	$<$1\% &	$<$1\% &	$<$1\% & $<$1\% & $<$1\% & $<$1\% \\

  \hline\hline

  \multirow{5}{*}{9} 
  
  & $\mathit{Constant}$ & $<$1\% &	$<$1\% &	1\% &	1\% &	1\% &	9\% &	- &	- &	- &	-\\
  & $\mathit{Edit}$ & $<$1\% &	$<$1\% &	$<$1\% &	1\% &	1\% &	7\% &	- &	- &	- &	-\\
  & $\mathit{DeepCoder}$ & $<$1\% &	$<$1\% &	1\% &	1\% &	1\% &	9\% &	- &	- &	- &	-\\
  & $\mathit{PCCoder}$ & $<$1\% &	$<$1\% &	$<$1\% &	1\% &	1\% &	7\% &	- &	- &	- &	-\\ 
  & $\mathit{\scheme_{FP}}$ & $<$1\% &	$<$1\% & 	$<$1\% &	$<$1\% &	4\% &	-  &	- &	- &	- &	- \\
  & $\mathit{\scheme_{LCS}}$ & $<$1\% &	$<$1\% &	$<$1\% &	$<$1\% &	3\% &	11\% &	17\% &	- &	- &	-\\
  & $\mathit{\scheme_{CF}}$ & $<$1\% &	$<$1\% &	1\% &	1\% &	1\% &	9\% &	- &	-  & - & 	- \\
  & $\mathit{\scheme_{LCS+Local search}}$ & $<$1\% &	$<$1\% &	$<$1\% &	3\% &	7\% &	16\% &	- &	- &	- &	-\\
  & $\mathit{\scheme_{CF+Local search}}$ & $<$1\% &	$<$1\% &	$<$1\% &	2\% &	5\% &	12\% &	- &	-  & - & 	- \\
  & $\mathit{Oracle_{LCS|CF}}$ & $<$1\% &	$<$1\% &	$<$1\% &	$<$1\% &	$<$1\% &	$<$1\% &	$<$1\% & $<$1\% & $<$1\% & $<$1\% \\

  \hline\hline

  \multirow{5}{*}{10} 
  & $\mathit{Constant}$ & $<$1\% &	1\% &	1\% &	90\% &	- &	- &	- &	- &	- &	-\\
  & $\mathit{Edit}$ & $<$1\% &	1\% &	1\% &	20\% &	43\% &	56\% &	- &	- &	- &	-\\
  & $\mathit{DeepCoder}$ & $<$1\% &	$<$1\% &	1\% &	9\% &	- &	- &	- &	- &	- &	-\\
  & $\mathit{PCCoder}$ & $<$1\% &	1\% &	1\% &	61\% &	- & - &	- &	- &	- &	-\\ 
  & $\mathit{\scheme_{FP}}$ & $<$1\% & 	$<$1\% &	$<$1\% &	4\% &	-  &	-  & - &	- &	- &	- \\
  & $\mathit{\scheme_{LCS}}$ & $<$1\% &	$<$1\% &	$<$1\% &	6\% &	16\% &	- &	- &	- &	- &	-\\
  & $\mathit{\scheme_{CF}}$ & $<$1\% &	$<$1\% &	1\% &	4\% &	12\% &	24\% &	-  &	- & - & 	- \\
  & $\mathit{\scheme_{LCS+Local search}}$ & $<$1\% &	$<$1\% &	$<$1\% &	6\% &	16\% &	- &	- &	- &	- &	-\\
  & $\mathit{\scheme_{CF+Local search}}$ & $<$1\% &	$<$1\% &	1\% &	4\% &	11\% &	24\% &	- &	-  & - & 	- \\
  & $\mathit{Oracle_{LCS|CF}}$ & $<$1\% &	$<$1\% &	$<$1\% &	$<$1\% &	$<$1\% &	$<$1\% &	$<$1\% & $<$1\% & $<$1\% & $<$1\% \\

  \hline\hline  
  \end{tabular} %}
  %}
% \end{minipage}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

In the experimental results section, we presented synthesis times for \scheme{} that included both GA time and NN-FF inferencing time.  Since inferencing time is significant, we speculate that further optimizations of our approach may be possible using futuristic deep learning accelerators~\cite{Shawahna:2019:ieee} that may eliminate some portion of the overall neural network inferencing time.
 Thus, we now show two versions of \scheme, the original non-optimized time, which includes the total wall clock time of \scheme\ with our hardware testbed environment, plus an optimized version after subtracting away inferencing time.  The results are presented in Table \ref{table:compare-extended}.

\begin{table*}[tpb]
  %\scriptsize
  %\parbox{0.3\linewidth}{
 % \begin{minipage}{\columnwidth}
  \centering
  \scalebox{0.9}{
  \begin{tabular}{clccccccccccc}
  \hline\hline
  \multirow{2}{*}{Program Length} & \multirow{2}{*}{MP System} & Synthesis & \multicolumn{10}{c}{Time Required to Synthesize (in seconds)} \\\cline{4-13}
  & & Percentage & 10\% & 20\% & 30\% & 40\% & 50\% & 60\% & 70\% & 80\% & 90\% & 100\%\\\hline\hline 
  
  \multirow{5}{*}{5}
  & $\mathit{DeepCoder}$ & 40\% & $<$1s & $<$1s & 2s & 126s & - & - & - & - & - &- \\
  & $\mathit{PCCoder}$ & 51\% & 1s & 1s & 6s & 66s & 357s & - & - & - & - & - \\ 
  & $\mathit{\scheme_{FP}}$ & 64\% & $<$1s & $<$1s & 4s & 174s & 525s & 803s & - & - & - & - \\  
  & $\mathit{\scheme_{FP}-Opt}$ & 64\% & $<$1s & $<$1s & 1s & 164s & 515s & 793s & - & - & - & - \\
  & $\mathit{\scheme_{LCS}}$ & 98\% & $<$1s & $<$1s & 4s & 43s & 112s & 349s & 600s & 690s & 838s & - \\
  & $\mathit{\scheme_{LCS}-Opt}$ & 98\% & $<$1s & $<$1s & 1s & 11s & 33s & 141s & 321s & 421s & 537s & - \\
  & $\mathit{\scheme_{CF}}$ &  96\% & $<$1s & $<$1s & 3s & 46s & 131s & 392s & 671s & 768s & 874s & - \\
  & $\mathit{\scheme_{CF}-Opt}$ &  96\% & $<$1s & $<$1s & 1s & 13s & 39s & 181s & 380s & 475s & 569s & - \\
  \hline\hline 
  
  \multirow{5}{*}{6} 
  & $\mathit{DeepCoder}$ & 45\% & $<$1s & $<$1s & $<$1s & 14s & - & - & - & - & - &- \\
  & $\mathit{PCCoder}$ & 75\% & 1s & 1s & 1s & 4s & 190s & 233s & 619s & - & - & - \\ 
  & $\mathit{\scheme_{FP}}$ & 63\% & $<$1s & $<$1s & 3s & 306s & 464s & 919s & - & - & - & - \\  
  & $\mathit{\scheme_{FP}-Opt}$ & 63\% & $<$1s & $<$1s & 1s & 296s & 457s & 909s & - & - & - & - \\
  & $\mathit{\scheme_{LCS}}$ & 87\% & $<$1s & $<$1s & 4s & 130s & 574s & 716s & 870s & 956s & - & - \\
  & $\mathit{\scheme_{LCS}-Opt}$ & 87\% & $<$1s & $<$1s & 1s & 56s & 307s & 429s & 579s & 658s & - & - \\
  & $\mathit{\scheme_{CF}}$ &  88\% & $<$1s & $<$1s & 3s & 183s & 533s & 732s & 872s & 918s & - & - \\
  & $\mathit{\scheme_{CF}-Opt}$ & 88\% & $<$1s & $<$1s & 1s & 66s & 281s & 435s & 569s & 612s & - & - \\
  \hline\hline 
  
  \multirow{5}{*}{7} 
  & $\mathit{DeepCoder}$ & 45\% & $<$1s & $<$1s & $<$1s & 13s & - & - & - & - & - &- \\
  & $\mathit{PCCoder}$ & 52\% & 1s & 1s & 2s & 11s & 635s & - & - & - & - & - \\ 
  & $\mathit{\scheme_{FP}}$ & 58\% & $<$1s & $<$1s & $<$1s & 393s & 566s & - & - & - & - & - \\  
  & $\mathit{\scheme_{FP}-Opt}$ & 58\% & $<$1s & $<$1s & $<$1s & 383s & 556s & - & - & - & - & - \\
  & $\mathit{\scheme_{LCS}}$ & 81\% & $<$1s & $<$1s & $<$1s & 176s & 676s & 1062s & 1134s & 1180s & - & - \\
  & $\mathit{\scheme_{LCS}-Opt}$ & 81\% & $<$1s & $<$1s & $<$1s & 92s & 445s & 775s & 834s & 886s & - & - \\
  & $\mathit{\scheme_{CF}}$ &  78\% & $<$1s & $<$1s & $<$1s & 127s & 609s & 889s & 956s & - & - & - \\
  & $\mathit{\scheme_{CF}-Opt}$ & 78\% & $<$1s & $<$1s & $<$1s & 49s & 349s & 593s & 655s & - & - & - \\
  \hline\hline

  \multirow{5}{*}{8} 
  & $\mathit{DeepCoder}$ & 56\% & $<$1s & $<$1s & $<$1s & $<$1s & 29s & - & - & - & - &- \\
  & $\mathit{PCCoder}$ & 57\% & 1s & 1s & 1s & 1s & 15s & - & - & - & - & - \\ 
  & $\mathit{\scheme_{FP}}$ & 49\% & $<$1s & $<$1s & $<$1s & 587s & - & - & - & - & - & - \\  
  & $\mathit{\scheme_{FP}-Opt}$ & 49\% & $<$1s & $<$1s & $<$1s & 577s & - & - & - & - & - & - \\
  & $\mathit{\scheme_{LCS}}$ & 68\% & $<$1s & $<$1s & $<$1s & 748s & 1545s & 1702s & - & - & - & - \\
  & $\mathit{\scheme_{LCS}-Opt}$ & 68\% & $<$1s & $<$1s & $<$1s & 571s & 1258s & 1401s & - & - & - & - \\
  & $\mathit{\scheme_{CF}}$ &  69\% & $<$1s & $<$1s & $<$1s & 404s & 988s & 1044s & - & - & - & - \\
  & $\mathit{\scheme_{CF}-Opt}$ & 69\% & $<$1s & $<$1s & $<$1s & 236s & 699s & 745s & - & - & - & - \\
  \hline\hline
  
  \multirow{5}{*}{9} 
  % this section will be updated. 
  & $\mathit{DeepCoder}$ & 53\% & $<$1s & $<$1s & $<$1s & $<$1s & 56s & - & - & - & - & -\\
  & $\mathit{PCCoder}$ & 55\% & 1s & 1s & 1s & 1s & 107s & - & - & - & - & - \\ 
  & $\mathit{\scheme_{FP}}$ & 52\% & $<$1s & $<$1s & $<$1s & $<$1s & 614s & - & - & - & - & - \\  
  & $\mathit{\scheme_{FP}-Opt}$ & 59\% & $<$1s & $<$1s & $<$1s & $<$1s & 605s & - & - & - & - & - \\
  & $\mathit{\scheme_{LCS}}$ & 64\%     & $<$1s & $<$1s & $<$1s &  1584s & 2544s & 2846s & - & - & - & - \\
  & $\mathit{\scheme_{LCS}-Opt}$ & 64\% & $<$1s & $<$1s & $<$1s &  1108s & 1704s & 2050s & - & - & - & -\\
  & $\mathit{\scheme_{CF}}$ &  67\%    & $<$1s & $<$1s & $<$1s & 837s & 1055s & 1195s & - & - & - & - \\
  & $\mathit{\scheme_{CF}-Opt}$ & 67\% & $<$1s & $<$1s & $<$1s & 489s & 744s & 798s & - & - & - & -\\
  \hline\hline
  
  
  \multirow{5}{*}{10}
  & $\mathit{DeepCoder}$ & 42\% & $<$1s & $<$1s & $<$1s & 67s & - & - & - & - & - & -\\
  & $\mathit{PCCoder}$ & 48\% & 1s & 1s & 1s & 1011s & - & - & - & - & - & - \\ 
  & $\mathit{\scheme_{FP}}$ & 49\% & $<$1s & $<$1s & $<$1s & 517s & - & - & - & - & - & - \\  
  & $\mathit{\scheme_{FP}-Opt}$ & 49\% & $<$1s & $<$1s & $<$1s & 507s & - & - & - & - & - & - \\
  & $\mathit{\scheme_{LCS}}$ & 55\% & $<$1s & $<$1s & $<$1s & 625s & 1640s & - & - & - & - & - \\
  & $\mathit{\scheme_{LCS}-Opt}$ & 55\% & $<$1s & $<$1s & $<$1s & 595s & 1523s & - & - & - & - & - \\
  & $\mathit{\scheme_{CF}}$ & 66\% & $<$1s & $<$1s & $<$1s & 164s & 957s & 1121s & - & - & - & - \\
  & $\mathit{\scheme_{CF}-Opt}$ & 66\% & $<$1s & $<$1s & $<$1s & 85s & 674s & 826s & - & - & - & - \\
 \hline\hline
  \end{tabular}}
  %\vspace{1cm}
  \caption{Comparison with DeepCoder and PCCoder in synthesizing different length programs. All experiments are done with the maximum search space set to 3,000,000 candidate programs.}
  \vspace{0.5cm}
  \label{table:compare-extended}
  %}
% \end{minipage}
\end{table*}

==> background.tex <==
%\section{Background}
\section{Previous work}
\label{sec-background}

%The goal of automatically generating software dates back to at least the 1950s~\cite{Backus:1957:FAC:IRE-AIEE-ACM}. However, there have been several technical challenges that have restricted a deeper exploration of MP when using only formally verified program synthesis techniques (e.g., proper program construction, effective pruning of the computational search space, data size and type limitations, etc.)~\cite{Gulwani:2011:popl, Solar-Lezama:2008:ucberkeley, Kamil:2016:pldi}.

%To address this, there has been a surge of research exploring machine programming using neural networks (NNs)~\cite{deepcoder, raychev14, bunel18, npi, cai17, real17, real18}. For example, DeepCoder~\cite{deepcoder} trains a DNN with input-output examples to predict the probabilities of the functions that are most likely to be used in a program. Raychev et al. take a different approach and use an \emph{n-gram} model (a technique that analyzes a contiguous sequence of elements) to predict the functions that are most likely to complete a partially constructed program~\cite{raychev14}. Bunel et al. explore a unique approach that combines reinforcement learning (RL) with a supervised model to find semantically correct programs~\cite{bunel18}. These are only a few of the research efforts in MP space using neural nets~\cite{npi, cai17}.

%As demonstrated by Becker and Gottschlich, genetic algorithms also show promise in MP~\cite{aip}. Google subsequently demonstrated that GAs can generate accurate image classifiers~\cite{real17, real18}. Their approach produced a state-of-the-art classifier for CIFAR-10~\cite{cifar10} and ImageNet~\cite{imagenet} benchmarks. Moreover, industrial research labs such as OpenAI, Uber Labs, Sentient Labs, and DeepMind have explored using evolutionary algorithms to automate the neural architecture optimization process~\cite{salimans17, such17, liu17, santientlabs}. 

%Unfortunately, even with this notable progress, GAs can be challenging to use due to the complexity of hand-crafting a GA's fitness function (FF). In this paper, we attempt to address this issue by automating the generation of the FF by representing its structure as a neural network, which we refer to as a neural network fitness function (NN-FF).

%We are not the first to propose such an approach. There are at least two prior works that have explored the automation of FFs using neural networks. Matos Dias et al. automated them for IMRT beam angle optimization, while Khuntia et al. used them for rectangular microstrip antenna design automation~\cite{Dias:2014:cejor, Bonomali:2005:motl}. At the highest level, these systems' automated NN-FFs behave as an approximation of a known mathematical model. 
%In essence, they act as a mathematical \emph{approximation} proxy. 

% We can't have the name NetSyn used here because it hasn't been defined yet.
%In contrast, our NN-FFs are fundamentally different in that we use a large corpus of program metadata (like DeepCoder) to train our NN-FFs to predict the likelihood that a given, incorrect solution will eventually converge to become a program generating the correct output.  
%This is because in the MP domain, we do not know the order of operations that would create the correct target program. As such, \scheme's NN-FFs predict the likelihood that a generated program will eventually converge on a correct one, whose generated output matches the given output. 
%We believe this approach to be the first of its kind automated \emph{prediction} FF for big data learning. 


% \am{Let me scribble some of my thoughts here. First, other works use NN as a way to approximate some rigorous mathematical models that are usually used to evaluate the quality of generated solutions. In that sense, NN acts more like a function approximator rather than a fitness predictor. Second, in MP domain, we do not know the actual target program. Therefore, fitness of a generated solution depends on the prediction of how similar the solution is to the target. So, this is a truly a prediction problem rather than an approximation problem. Our use of NN essentially maps this prediction problem into big data learning problem.}







==> impact.tex <==
\section*{Broader Impact}
Constructing fitness functions automatically based on example solutions holds immense potential in making genetic algorithms more effective and enhancing their applicability. This paper demonstrates how such a fitness function can be used to
synthesize programs autonomously based on specifications. 
The proposed solution offers an approach competitive to the state-of-the-art program synthesis techniques.  
This type of fitness function can enable genetic algorithms to offer better solutions in other applications such as finding better ML models, finding new chemical molecules with certain properties without detailed chemical simulation,
finding code-breaking ciphers quickly, configuring hardware and software for a particular goal, construction of facial composites in forensic science etc.


We note that with our techniques and other program synthesis systems that some of the burden of software development can be removed from programmers, allowing them to be more productive by on average focusing on higher-level and more creative aspects of their software systems.  With the current shortage of computer programmers expected to continue into the future, techniques that allow parts of the software development life cycle to be automated offer hope that the effects of this programmer shortage can be somewhat mitigated through increases in existing programmer productivity. Moreover, these techniques can help novice programmers by providing close-complete code at least for some simple tasks.

%Such synthesis techniques can enable ease of programmingand subsequent adoption of the future computing platforms.  Future platforms will be heterogeneous withdifferent types of CPUs, GPUs, accelerators, FPGAs, etc.  This project offers an innovative programmingand development model that can automate complete or partial development of software code for heteroge-neous platforms.  The proposed ideas can help generate different versions of code implementing the samefunctionalities.  This type of versioning capabilities are key enablers for self-aware computing in exascalesystems. Similarly, the proposed autonomous programming techniques can be used to synthesize proxy ap-plications that have similar behavior as the larger more complex applications. Proxy applications are widelyused in DOE labs for reliability analysis [15].  More details about the impact of this project to DOE can befound in Section 5

==> intro.tex <==
% !TEX root = main.tex
\section{Introduction}
\label{sec-intro}
% Intro to MP and program synthesis
In recent years, there has been notable progress in the space of automatic software generation, also known as \emph{Machine Programming} (MP)~\cite{gottschlich:2018:mapl, ratner:2018:sysml}. MP can be achieved in many ways. One way is by using \emph{formal program synthesis}, a technique that uses formal methods and rules to generate programs~\cite{mana75}. Formal program synthesis usually guarantees some program properties by evaluating a generated program's semantics against a corresponding specification~\cite{gulwani12, alur15}. Although useful, such formal synthesis techniques can often be limited by exponentially increasing computational overhead that grows 
%proportionally 
with the program's instruction size~\cite{Heule:2016:pldi, Bodik:2013:sttt, Solar-Lezama:2006:asplos, Loncaric:2018:icse, Cheung:2012:cikm}.

% MP with ML - probabilistic correctness
An alternative to formal methods for MP is to use machine learning (ML). Machine learning differs from traditional formal program synthesis in that it generally does not provide correctness guarantees. Instead, ML-driven MP approaches are usually only \emph{probabilistically} correct, i.e., their results are derived from sample data relying on statistical significance~\cite{Murphy:2012:mitpress}. Such ML approaches tend to explore software program generation using an objective function. Objective functions are used to guide an ML system's exploration of a problem space to find a solution. 
%An alternative to formal methods for MP is to use machine learning (ML)~\cite{deepcoder, raychev14, bunel18, npi, cai17, aip, real17, real18}. Machine learning differs from traditional formal program synthesis in that it generally does not provide correctness guarantees. Instead, ML-driven MP approaches are usually only \emph{probabilistically} correct, i.e., their results are derived from sample data relying on statistical significance~\cite{Murphy:2012:mitpress}. Such ML approaches tend to explore software program generation using an objective function. Objective functions are used to guide an ML system's exploration of a problem space to find a solution. %For example, \emph{backpropagation}, the objective function used in deep neural networks (DNNs), is a gradient-based optimization algorithm that aims to iteratively reduce the error of the DNN using mathematical differentiation~\cite{Rumelhart:1986:nature}. 

% Prior work on ML for MP
%\jt{Please can someone confirm that the citations in this paragraph are NN-based? A few of these, like Real et al. are cited as GA methods as well.}
More recently, there has been a surge of research exploring ML-based MP using neural networks (NNs). For example, in \cite{deepcoder}, the authors train a neural network with input-output examples to predict the probabilities of the functions that are most likely to be used in a program. Raychev et al.~\cite{raychev14} take a different approach and use an n-gram model %(a technique that analyzes a contiguous sequence of elements) 
to predict the functions that are most likely to complete a partially constructed program.
Robustfill~\cite{robustfill} encodes input-output examples using a series of 
recurrent neural networks (RNN), and generates the the program using another RNN one token at a time.
Bunel et al.~\cite{bunel18} explore a unique approach that combines reinforcement learning (RL) with a supervised model to find semantically correct programs. These are only a few of the works in the MP space using neural networks~\cite{npi, cai17, Chen18}.

% GA for MP
%Objective functions can also come in the form of heuristics, which are commonly used in genetic algorithms (GAs). A \emph{genetic algorithm} is a machine learning technique that attempts to solve a problem from a pool of candidate solutions. These generated candidates are iteratively evolved and mutated after qualifying from various grading criteria. The primary grading system used in genetic algorithms is the \emph{fitness function}. Fitness functions are usually hand-crafted heuristics that grade the approximate correctness of candidate solutions. 

As demonstrated by Becker and Gottschlich~\cite{aip}, genetic algorithms also show promise for MP. 
Significant research has been done in the field of genetic programming~\cite{stackgp, lgp, allgp} whose goal is to find a solution in the form of a complete or partial program for a given specification. Existing techniques focus either on representation of programs or operators during the evolution process. 
Real et al.~\cite{real18} recently demonstrated that genetic algorithms can generate accurate image classifiers. Their approach produced a state-of-the-art classifier for CIFAR-10~\cite{cifar10} and ImageNet~\cite{imagenet} datasets. Moreover, genetic algorithms have been exploited to successfully automate the neural architecture optimization process~\cite{salimans17, such17, liu17, santientlabs, real2020automlzero}. Even with this notable progress, genetic algorithms can be challenging to use due to the complexity of hand-crafting fitness functions that guide the search. 

% This work
While genetic algorithms have had demonstrable success in their practical applications~\cite{Korns2011, such17, Read:2018:dblp}, an open challenge is in creating simple, yet effective fitness functions. An impediment to this goal is that fitness function complexity tends to increase proportionally with the problem being solved. In this paper, we explore an approach to automatically generate these fitness functions by representing their structure with a neural network, making the following technical contributions:
\begin{itemize}
%\setlength\itemsep{0.25em}
    \item {\em Fitness Function:} Our fundamental contribution is in the automation of fitness functions for genetic algorithms. We propose to do so by mapping fitness function generations as a big data learning problem. To the best of our knowledge, our work is the {\em first} of its kind to use a neural network as a genetic algorithm's fitness function for the purpose of MP. 
    %Moreover, the neural network provides additional insights that can be exploited to better mutate the genes of genetic algorithms .
    
    \item {\em Convergence:} A secondary contribution is in our utilization of local neighborhood search to improve the convergence of approximately correct candidate solutions. We demonstrate its efficacy empirically.
    % We propose two such approaches and demonstrate their efficacy in a number of benchmarks. 
    
    \item {\em Generality:} We demonstrate that our approach can support different neural network fitness functions, uniformly. We develop a neural network model to predict the fitness score based on the given specification and program trace.
%While our experiments are strictly in the space of MP, we are not aware of any restrictions from utilizing our fitness function automation technique in other domains.
    
    \item {\em Metric:} We contribute a new metric suitable for MP domain. The metric, ``search space'' size (i.e., how many candidate programs have been searched), is an alternative to program generation time, and is designed to emphasize the algorithmic efficiency as opposed to the implementation efficiency of an MP approach.
    
    %While prior work~\cite{deepcoder,Zohar:2018:nips} aims at optimizing program generation time, we argue that program generation time does not fully capture the efficiency of the generation algorithm. Instead, it captures implementation efficiency of the algorithm. %To capture the efficiency of the generation algorithm itself, 
    %Therefore, we propose to use ``search space'' size, i.e., how many candidate programs have been searched, as an alternative metric and demonstrate its value for comparing MP approaches.
\end{itemize}

%While GAs have had demonstrable success in their application in both research and industrial communities~\cite{Korns2011, such17, Read:2018:dblp}, an open challenge is in creating simple, yet effective fitness functions. Contrary to this goal, fitness function complexity tends to increase proportionally with the problem being solved. In this paper, we explore an approach to automatically generate these fitness functions, making the following technical contributions:

%In this paper, we attempt to address this issue by automating the generation of the FF by representing its structure as a neural network, which we refer to as a neural network fitness function (NN-FF).
%We are not the first to propose such an approach. There are at least two prior works that have explored the automation of FFs using neural networks. Matos Dias et al.~\yrcite{Dias:2014:cejor} automated them for IMRT beam angle optimization, while Khuntia et al.~\yrcite{Bonomali:2005:motl} used them for rectangular microstrip antenna design automation. At the highest level, these automated NN-FFs behave as an approximation of a known mathematical model. %In essence, they act as a mathematical \emph{approximation} proxy. 

%In contrast, our NN-FFs are fundamentally different in that we use a large corpus of program metadata (like DeepCoder) to train our NN-FFs to predict the likelihood that a given, incorrect solution will eventually converge to become a program generating the correct output.  
%This is because in the MP domain, we do not know the order of operations that would create the correct target program. As such, \scheme's NN-FFs predict the likelihood that a generated program will eventually converge on a correct one, whose generated output matches the given output. 
%We believe this approach to be the first of its kind automated \emph{prediction} FF for big data learning. 

%In Section~\ref{sec-background}, we briefly describe related work. In Section~\ref{sec-problem}, we describe the general problem statement and the way we constrain it. In Section~\ref{sec-main}, we discuss the \scheme\ framework. 
%In Section~\ref{sec-lessons}, we discuss lessons learned. 
%In Section~\ref{sec-results}, we describe our experimental results and in Section~\ref{sec-conc} we conclude.





==> observations.tex <==



\subsection{Observations}
\label{sec-lessons}

During the course of this project, we attempted to extend \scheme\ with several ideas. 
Not all worked out. The failed attempts along with some explanation 
%of the failures 
are as follows: 

    %\item 
    {\em 3. Multiple predictors:} 

        %\item {\em }
%\end{itemize}
%\end{enumerate}

==> old_design.tex <==
% overview
% Encoding
% Crossover \& Mutation
% Fitness function:
% - CF
% - LCS
% - Deepcoder
% Neighborhood search:
% - parametric neighborhood search
% - BFS
% - DFS
% In implementation/result section, talk about training data generation


\section{\scheme: Program Synthesis Framework}
\label{sec-main}

In this section, we describe \scheme's design as illustrated in Figure~\ref{fig-overview}.

\scheme\ 
starts with input-output examples $S^{t_o}_{t_i}$ for the target program $P^t$ to be synthesized and a set of training programs (Figure~\ref{fig-overview}).  
First, \scheme\ uses a process described in Section~\ref{sec-fitness} to transform the training programs into a set of input-output examples $S^{e_o}_{e_i}$ on which a neural network is trained.  
This process needs only be done once and \scheme\ can then use the resulting model as a fitness function
%to predict fitness scores of genes 
to synthesize multiple target programs.
%a training set of input-output examples and corresponding programs as well as
%some input-output examples of the program to be synthesized (i.e., target program). A neural network is trained with the training set. 
%This trained neural network is used in the evolutionary algorithm to predict fitness scores of genes. 
Next, \scheme\ creates a population of random genes (i.e., candidate programs) of a given length and uses the neural network model to estimate the fitness of each gene.  Higher performing genes are preferentially selected for crossover and mutation to produce the next generation of genes.  The genetic algorithm iterates from one generation to the next in this manner
until \scheme\ finds the target program as verified by the input-output examples. From time to time, \scheme\ takes the top $N$ scoring genes from the population, determines the neighborhood of those genes and searches for the target program there. If the target program is not found, \scheme\ continues with the genetic algorithm.  The following sections provide a description of each component. Details of the genetic algorithm such as population size and mutation frequency can be found in Appendix~\ref{sec-appendix-system}.

\begin{figure}[htpb]
\begin{center}
\includegraphics[width=1.05\linewidth]{./FIGS/Overview_new}%\vspace{-0.1cm}
%\includegraphics[width=0.85\linewidth]{./FIGS/Overview_cropped}%\vspace{-0.2cm}
\caption{Overview of \scheme}
\label{fig-overview}
\end{center}
\vspace{-0.6cm}
\end{figure}

\subsection{Gene Encoding}
\label{sec-encoding}
\scheme\ uses value encoding approach where a gene 
%(i.e., a candidate program) 
$\zeta$ is represented as a sequence 
of values $[C:C\in \{x\}^{|\Sigma_{DSL}|}_{x=1}]$ where $\Sigma_{DSL}$ is the set of 
functions from our DSL.
$C$ can be thought of as an id corresponding to one of the DSL functions. 
This encoding makes it easier to implement crossover and mutation without generating any invalid gene.

\subsection{Crossover \& Mutation}
\label{sec-cross}
\scheme\ starts with a randomly initialized gene population. To form the next generation during the genetic algorithm, a small percentage (e.g., 20\%) of top performing genes are copied into the next generation unmodified to guarantee that top performers are preserved.  The remaining genes are created through crossover or mutation with some probability. For crossover, two genes are selected using Roulette Wheel algorithm with the crossover point selected randomly.
%For a particular gene $\zeta$, crossover is done between $\zeta$ and some other gene
%selected using the Roulette Wheel algorithm with the crossover point selected randomly. 
For mutation, one gene is Roulette selected and the mutation point in that gene is selected randomly.  The selected value $C$ is mutated to some other random value $C'$ such that 
$C'\in \{x\}^{|\Sigma_{DSL}|}_{x=1}$ and $C'\ne C$. Crossover and mutation can 
sometimes lead to a new gene with dead code. \scheme\ checks for dead code (Section ~\ref{dead_code_elimination}). If dead code is present, \scheme\  repeats crossover and mutation until a gene without dead code is produced.  

\subsection{Dead Code Elimination}
\label{dead_code_elimination}

Dead code elimination (DCE) is a classic compiler technique to remove code from a program which has no effect on the program's output.  Such dead code is possible in our list DSL if the output of a statement is never used.  We implemented DCE in \scheme\ by tracking the input/output dependencies between statements and eliminating those statements whose outputs are never used.  \scheme\ uses DCE during candidate program generation and during crossover/mutation to make sure that the effective length of the program is not less than the target program length due to the presence of dead code.

\subsection{Neural Network Based Fitness Function}
\label{sec-fitness}

To determine the fitness of a gene $\zeta_g=[C_g]$ generated during the genetic algorithm, \scheme\ executes the gene with inputs $I^t$, producing an input-output set $S^{g_o}_{t_i}$.
The goal of the fitness function is to estimate the quality of $\zeta_g$ by using a combination of $S^{g_o}_{t_i}$ and $S^{t_o}_{t_i}$. A higher fitness
score implies a higher quality gene (i.e., one closer to the target).

\scheme\ uses a trained neural network model as a fitness function.  
%Since predictions on this model will be made with input $S^{g_o}_{t_i}$, the model must similarly be trained on some set $S^{e_o}_{e_i}$. 
For training the neural network, \scheme\ uses a set of randomly generated example programs $E$.
%When \scheme\ is given a set $E$ of example programs, 
 \scheme\ generates a random set of inputs $I^e$ for each program in $P^e$ in $E$, executes $P^e$ with those inputs, and calculates the outputs.
%the associated quality metric (see below)
%Sections ~\ref{sec-cf}, ~\ref{sec-lcs}).  
%This collection of inputs and outputs from the programs in set $E$ is called $S^e_e$. 
For each $P^e$ in $E$, \scheme\ takes a randomly generated program $P^r$ (not from $E$),
%for each example program from $E$, 
apply
the previously generated inputs (corresponding to $P^e$) to $P^r$ to get outputs ($O^r$), and compare the $P^r$ with $P^e$
to calculate quality metrics (see below). 
%The collection of of all 
%inputs and outputs from this process forms the set $S^e_e$.
%Then, \scheme\ will take subsets of each program, omitting one statement (i.e, introducing a bug), run those subsets on the same inputs, and again calculate the associated quality metrics.  \scheme\ repeats this process with smaller and smaller subsets until subset length is 1.  \scheme\ also generates unrelated random programs with minimal quality metrics to act as negative training examples.
%The collection of all the inputs and outputs from this process forms the set $S^e_e$.
%Since there are more possible program subsets closer to half the program length, \scheme\ uses a random filtering scheme to make sure that each quality metric is approximately equally represented in $S^e_e$ so that the training cannot minimize loss by always outputting the same value.
%%and each entry in this set is mapped to the associated quality metric.  
%\scheme\ then trains the neural network to associate its input with the associated quality metrics.
\scheme\ trains the neural network to learn the quality metrics.
The inputs for the neural network can be chosen from several options: (i) $S^{r_o}_{e_i}$ only, which we call the $IO$ model, (ii) $S^{e_o}_{e_i}$ and $S^{r_o}_{e_i}$, which we call the $IO^2$ model and (iii) the difference between the inputs and outputs in $S^{e_o}_{e_i}$ and $S^{r_o}_{e_i}$, which we call the $IO^\delta$ model.
In this way, the network is trained on a variety of program correctness levels, from totally correct to totally incorrect. During inference time, each generated candidate program $P^g$
behaves like $P^r$
%those randomly generated programs 
and the target program $P^t$ behaves like $P^e$. 
%the example programs. 
Therefore, $IO$ model takes inputs from $S^{g_o}_{t_i}$ during inference.
Similar is the case for $IO^2$ and $IO^\delta$ models.
%model will take inputs from $S^$
%Let us assume that our target program can be represented by gene $\zeta_t=[C_t]$. \scheme\
%has been provided with a set of input-output examples $\{(I^t_j, O^t_j)\}^n_{j=1}$ for 
%$\zeta_t$ as well as a training set $T$. 
%Let us assume that a gene $\zeta_g=[C_g]$ is generated during the 
%evolutionary algorithm, and it produces input-output examples $\{(I^t_j, O^g_j)\}^n_{j=1}$.
%The goal of the fitness function is to estimate the quality of $\zeta_g$. Higher fitness
%score implies higher quality gene (i.e., the gene is close to the target).
Details of how we trained the neural network can be found in Appendix~\ref{sec-appendix-system}.

%The central component of an evolutionary algorithm is its fitness function. 
We can contrast \scheme 's fitness function with a more commonly used fitness function based on edit distance, where the score of gene $\zeta_g$ is the
edit distance between $[O^t_j]^n_{j=1}$ and $[O^g_j]^n_{j=1}$. We have found that such an edit distance-based fitness function 
%usually 
leads to poor 
results for the synthesis process (e.g., target programs may be found only one-third of the time when compared to \scheme 's fitness function).
%The poor results are caused by the fact that edit distance only considers outputs as an indication of quality of $\zeta_g$, not the actual gene itself. 
Thus, \scheme\ uses its trained neural network %Therefore, we propose to use a neural network that will use $[I^t_j]^n_{j=1}$,
%$[O^t_j]^n_{j=1}$ and $[O^g_j]^n_{j=1}$ 
to predict the {\em quality} of $\zeta_g$ 
with respect to $\zeta_t$.
Essentially, the design of a fitness function is mapped to a big data problem where a 
neural network will learn to predict the quality of gene by training on programs from $E$. 
We design three quality metrics and compare their performance in synthesizing programs.
%We compare our two quality metrics  against another quality metric (Function Probabilty) proposed in Deepcoder.

%\subsubsection{Common Functions}
%\label{sec-cf}
\paragraph{Common Functions}
\scheme\ can use the number of common functions (CF) between $\zeta_g$ and $\zeta_t$ as a 
quality metric for $\zeta_g$. In other words, the fitness score of $\zeta_g$ is $f^{CF}_{\zeta_g}=|\mathbf{elems}~\zeta_g \cap \mathbf{elems}~\zeta_t|$.
\scheme\ constructs training data for $f^{CF}$ from $E$ as described in Section ~\ref{sec-fitness} and feeds to a neural network for 
training. 
 Since the output
of the neural network will be an integer from 0 to $\mathbf{len}~\zeta_t$, the 
neural network can be designed as a multiclass classifier with a softmax layer as the final
layer.
%have several options for inputs of the neural network. 
%For example, we can consider input
%and output from candidate gene ($IO$ model) as neural network inputs. Alternatively,
%we can consider input and output from both target and 
%candidate
%gene ($IO^2$ model) as neural network inputs. Finally, we can also consider the difference between input and target's output and difference between
%input and candidate's output ($IO^\delta$ model) as neural network inputs. Our experimental
%results show that $IO$ model allows \scheme\ to find programs more frequently (Section~\ref{sec-results}).

%\subsubsection{Longest Common Subsequence}
\paragraph{Longest Common Subsequence}
\label{sec-lcs}
\scheme\ can use longest common subsequence (LCS) between $\zeta_g$ and $\zeta_t$ as
an alternative to CF. So, the fitness score of $\zeta_g$ is 
$f^{LCS}_{\zeta_g}=\mathbf{len}~LCS(\zeta_g, \zeta_t)$. Similar to CF,
training data can be constructed from $E$ which is then fed into a multiclass classifier
neural network. 
%Inputs of the neural network can be $IO$ or $IO^2$ or $IO^\delta$.

\paragraph{Function Probability}
%\subsubsection{Function Probability}
\label{sec-deep}
DeepCoder~\cite{deepcoder} proposed 
%to generate 
a probability map for the functions in DSL. We can construct a quality metric
using the probability map. Let us assume that the probability map is 
$[p_i:p_i=P(C_i\in \mathbf{elems}~\zeta_t|\{(I^t_j, O^t_j)\}^n_{j=1})]^{|\Sigma_{DSL}|}_{i=1}$. 
A multiclass multilabel classifier neural network with sigmoid layer as the last layer can be used to predict the probability map. Training data
can be constructed for the neural network using $E$. \scheme\ can use
the probability map to calculate the fitness score of $\zeta_g$ as
$f^{FP}_{\zeta_g}=\Sigma (p_i:C_i \in \mathbf{elems}~\zeta_g)$.
\scheme\ can even use the probability map to guide the mutation process.
For example, instead of mutating a function $C$ with $C'$ that is 
selected randomly, \scheme\ can select $C'$ using Roulette Wheel
algorithm using the probability map.
%where individual $p_i$

%\begin{wrapfigure}{r}{0.4\linewidth}
\begin{figure}[htpb]
\begin{center}
\includegraphics[width=0.6\columnwidth]{./FIGS/NS}
%\vspace{-0.2cm}
\caption{Neighborhood for a $4$ length gene using (a) BFS and (b) DFS based approach.}
\label{fig-neighborhood}
\end{center}
\vspace{-0.4cm}
\end{figure}
%\end{wrapfigure}


\subsection{Neighborhood Search}
\label{sec-neighbor}
Neighborhood search (NS) checks some candidate
genes in the {\em neighborhood} of the $N$ top scoring genes from the genetic
algorithm. The rationale is that if the target gene $\zeta_t$ is in that 
neighborhood, \scheme\ can quickly find it without relying on the genetic
algorithm. 
%\scheme\ needs to decide when to invoke NS and how to define the neighborhood.




%\subsubsection{When to Invoke NS?}
%\label{sec-invoke}
\paragraph{When to Invoke NS?}
If \scheme\ has finished $l$ generations so far,
%is about to start $l+1$ generation. 
$\mu_{l-w+1,l}$ will denote the average fitness score of
genes for the last $w$ iterations (i.e., from $l-w+1$ to $l$ iterations)
and $\mu_{1,l-w}$ denotes the average fitness scores before the last $w$ iterations 
(i.e., from $1$ to $l-w$ iterations). Here, $w$ is the sliding window. \scheme\
invokes NS if $\mu_{l-w+1,l} \le \mu_{1,l-w}$. The rationale is that \scheme\ is not
producing improved genes for the last $w$ iterations (i.e., saturating) and therefore, 
should check if the neighborhood contains $\zeta_t$.

%\subsubsection{How to Define Neighborhood?}
%\label{sec-neighbor-define}
\paragraph{How to Define Neighborhood?}
Algorithm~\ref{algo-neighbor} shows how to define and search a neighborhood.
The algorithm is inspired by the principle of breadth first search (BFS).
%based on the BFS approach. 
For each top scoring gene $\zeta_g$, \scheme\ considers one function at a time
starting from the first function of the gene to the last one. For each selected functionm
\scheme\
replaces that function with all other functions from $\Sigma_{DSL}$, and inserts
the resultant genes into the neighborhood set $N$. If $\zeta_t$ is found in $N$, \scheme\ 
stops there by returning the solution. Otherwise, it continues the search and returns to 
the genetic algorithm. The complexity of the search is
$\mathcal{O}(N\times \mathbf{len}~\zeta_g\times|\Sigma_{DSL}|)$ which is significantly 
smaller than the exponential search space used by a traditional BFS algorithm.
%that of a typical exhaustive search such as BFS.



%%%%%%%%%% Need to use a different package
\begin{algorithm}
\small
\KwIn{A set $G$ of top $N$ scoring genes from last generation}
\KwOut{$\zeta_t$ if found}
\For{Each $\zeta_g \in G$}{
  $N \gets \emptyset$
  
  \For{$i \gets 1~\mathbf{to~len}~\zeta_g$}{
    \For{$j \gets 1~\mathbf{to} |\Sigma_{DSL}|$}{
      $\zeta_n \gets \zeta_t~with~\zeta_t[i]~replaced~with~C_j$
      $~~such~that~\zeta_t[i] \ne C_j$
      
      $N \gets N \cup \zeta_n$
    }
  }
  Check if $\zeta_t \in N$
  
  \Return{$\zeta_t$ if found}
}
\Return{}
\caption{Defines and searches neighborhood based on BFS principle}
\label{algo-neighbor}
\end{algorithm}

Similar to BFS, \scheme\ can define and search the neighborhood using an approach similar to
depth first search (DFS). It
is similar to Algorithm~\ref{algo-neighbor} except $i$ will keep track of depth here.
After the loop in line 4 finishes, \scheme\ needs to pick the best scoring gene from $N$
to replace $\zeta_g$ before going to the next level of depth. The algorithmic complexity 
will remain the same. Figure~\ref{fig-neighborhood} shows examples of neighborhood 
using BFS and DFS based approach.




%\begin{algorithm}
% \KwIn{A set $C = \{c_1, c_2, \ldots, c_r\}$ of denominations of coins, where $c_i > c_2 > \ldots > c_r$ and a positive number $n$}
%\KwOut{A list of coins $d_1,d_2,\ldots,d_k$, such that $\sum_{i=1}^k d_i = n$ and $k$ is minimized}
%$C \gets \emptyset$
%\For{$i \gets 1$ \textbf{to} $r$}{
%  \While{$n \geq c_i$} {
%    $C \gets C \cup \{c_i\}$\;
%    $n \gets n - c_i$\;
%  }
%}
%\Return{$C$}\;
%\caption{Decides when to invoke NS}
%\label{algo:NS}
%\end{algorithm}

%\subsubsection{BFS Based Neighborhood}
%\subsubsection{DFS Based Neighborhood}

==> old_text_justin.tex <==





\newpage


There are at least two primary hurdles in using evolutionary algorithms to synthesize programs.
{\em First}, it is non-trivial to design appropriate fitness functions.
Without a proper fitness function, an evolutionary algorithm may take a long time to (or never) converge. 

{\em Second}, evolutionary algorithms are often quick to find {\em close-enough} solutions but program synthesis requires exact solutions, which may take much longer to find. To address these 
challenges, we make two novel contributions. {\em First}, we use a neural network to automatically discover a suitable fitness function. The neural network determines which properties of candidate programs (i.e., \emph{genes} in evolutionary algorithm terminology) should be used as the fitness score.
In essence, we cast the design of a fitness function as a big data problem where a 
neural network learns to predict the quality of a gene by training on example programs.
{\em Second}, to move from approximate to precise program solutions, we occasionally check the local program space (i.e., {\em the neighborhood}) of some top scoring genes to search for an exact solution. Thus, we combine an evolutionary algorithm with occasional neighborhood
search to expedite the convergence process.

We have implemented these contributions in a framework, called {\em \scheme}, that 
synthesizes programs using an evolutionary algorithm. \scheme\ trains a neural network with
a set of programs (and their input-output examples) to predict various properties of those programs. We experimented with two different properties and compared 
their performance against Deepcoder's function probability based fitness score. Our results showed that \scheme\ performs better than Deepcoder's approach (e.g., $\mathbf{1.8\times}$ more synthesis rate).

The paper makes the following contributions:
\begin{itemize}
    \item {\em Fitness Function:} We make a fundamental contribution in automating the design of fitness functions for evolutionary algorithms.
    %used in evolutionary algorithm. 
    To the best of our knowledge, \scheme\ is the {\em first} work that uses a neural network as the fitness function in an evolutionary algorithm.
    
    \item {\em Convergence:} \scheme\ is the {\em first} work that uses {\em neighborhood} search to improve the convergence process of evolutionary algorithms. We propose two approaches to determine the {\em neighborhood} search space.
    
    \item {\em Generality:} We implement an end-to-end program synthesis framework 
    \scheme\ and demonstrate that \scheme\ can support different neural network fitness functions uniformly.
    
\end{itemize}

For the rest of this paper, we \emph{(i)} formalize the problem we are trying to solve, \emph{(ii)} describe our proposed solution, and \emph{(iii)} discuss failed attempts and the lessons learned from those efforts. We then present experimental results and draw some initial conclusions.





\newpage



%For example, DeepCoder trains a DNN with input-output examples to predict probabilities of the functions that are most likely to be used in a program~\cite{deepcoder}. Raychev et al. use an \emph{n-gram} model, which analyzes a contiguous sequence of elements, to predict those functions most likely to complete a partial program~\cite{raychev14}. Bunel et al. use reinforcement learning (RL) in conjunction with a supervised model to find semantically correct programs~\cite{bunel18}. Besides these, there are many other research efforts in the space of machine programming using neural networks~\cite{npi, cai17}.

%certain properties of a program (e.g., probability of having a certain function). 
%The predicted probabilities can be used in an SMT solver or an enumerative search technique to find the program quickly. 

%Neo extends Deepcoder to include information about
%conflicting functions during the synthesis process~\cite{feng18}. 

%Despite the significant strides,
%%in the domain of program synthesis, 
%there is little or no effort in using evolutionary (i.e., genetic) algorithms to synthesize programs. 



As demonstrated by Becker and Gottschlich, genetic algorithms also show promise in MP~\cite{aip}.


With the heightened interest in deep learning, less attention has been given to using evolutionary (i.e., genetic) algorithms for program synthesis. Yet, evolutionary algorithms are a promising approach to solve complex problems, showing notable success in many challenging areas. For example, Google
uses evolutionary algorithms to find the most accurate image classifiers~\cite{real17, real18}. Their approach produced the state-of-the-art classifier for CIFAR-10~\cite{cifar10} and ImageNet~\cite{imagenet} benchmarks. Moreover, leading research labs such as OpenAI, Uber Labs, Sentient Labs and DeepMind use evolutionary algorithms to automate the neural architecture optimization process~\cite{salimans17, such17, liu17, santientlabs}. However, applications of evolutionary algorithms for program synthesis have been limited to finding mutual exclusion algorithms~\cite{katz08}, repairing bugs~\cite{weimer09}, and writing code in a primitive language called BF~\cite{aip}.

%(more details are in Section~\ref{sec-rel}).
%Despite the significant strides,
%%in the domain of program synthesis, 
%there is little or no effort in using evolutionary algorithm to synthesize 
%programs. This is surprising given the fact that evolutionary algorithm is inherently parallel, has the potential to find solutions quickly, and 
%accommodates different objective functions easily.
%Part of the challenge 

%The lack of interest in the evolutionary approach to synthesize programs is primarily caused by two major challenges. 

There are at least two primary hurdles in using evolutionary algorithms to synthesize programs.
{\em First}, it is non-trivial to design appropriate fitness functions.
Without a proper fitness function, an evolutionary algorithm may take a long time to (or never) converge. 
{\em Second}, evolutionary algorithms are often quick to find {\em close-enough} solutions but program synthesis requires exact solutions, which may take much longer to find. To address these 
challenges, we make two novel contributions. {\em First}, we use a neural network to automatically discover a suitable fitness function. The neural network determines which properties of candidate programs (i.e., \emph{genes} in evolutionary algorithm terminology) should be used as the fitness score.
In essence, we cast the design of a fitness function as a big data problem where a 
neural network learns to predict the quality of a gene by training on example programs.
{\em Second}, to move from approximate to precise program solutions, we occasionally check the local program space (i.e., {\em the neighborhood}) of some top scoring genes to search for an exact solution. Thus, we combine an evolutionary algorithm with occasional neighborhood
search to expedite the convergence process.

We have implemented these contributions in a framework, called {\em \scheme}, that 
synthesizes programs using an evolutionary algorithm. \scheme\ trains a neural network with
a set of programs (and their input-output examples) to predict various properties of those programs. We experimented with two different properties and compared 
their performance against Deepcoder's function probability based fitness score. Our results showed that \scheme\ performs better than Deepcoder's approach (e.g., $\mathbf{1.8\times}$ more synthesis rate).

The paper makes the following contributions:
\begin{itemize}
    \item {\em Fitness Function:} We make a fundamental contribution in automating the design of fitness functions for evolutionary algorithms.
    %used in evolutionary algorithm. 
    To the best of our knowledge, \scheme\ is the {\em first} work that uses a neural network as the fitness function in an evolutionary algorithm.
    
    \item {\em Convergence:} \scheme\ is the {\em first} work that uses {\em neighborhood} search to improve the convergence process of evolutionary algorithms. We propose two approaches to determine the {\em neighborhood} search space.
    
    \item {\em Generality:} We implement an end-to-end program synthesis framework 
    \scheme\ and demonstrate that \scheme\ can support different neural network fitness functions uniformly.
    
\end{itemize}

For the rest of this paper, we \emph{(i)} formalize the problem we are trying to solve, \emph{(ii)} describe our proposed solution, and \emph{(iii)} discuss failed attempts and the lessons learned from those efforts. We then present experimental results and draw some initial conclusions.

%In Section ~\ref{sec-problem} we formalize the problem we are solving.  In Section ~\ref{sec-desc} we describe our solution to the problem.  Lessons learned are discussed in Section ~\ref{sec-lessons}.  Results are presented in Section ~\ref{sec-results} and comparisons made to related work in Section ~\ref{sec-rel}.  Finally, we draw conclusions in Section ~\ref{sec-conc}.

%For a given gene, the neural 
%network predicts properties such as how many functions might be common between this gene 
%and the solution or what is

%partly caused by the difficulty in finding appropriate fitness function. To overcome this %difficulty, this paper contributes with a novel approach 
%%to design fitness functions, 
%which is to use a neural network
%as a fitness function. Based on this idea, we propose an evolutionary framework to synthesize %program. The framework, called ESP, contains three novel contributions. 
%Among various machine learning
%bases synthesis techniques, Neural Program Synthesis
%techniques are particularly interesting because such
%techniques can produce actual programs by conditioning a neural network with input-output examples~\cite{}.

%Machine learning based program synthesis can be broadly categorized as Neural Program Induction techniques and Neural Program Synthesis technqiues. Neural Program Induction techniques~\cite{} strive to design a neural network that learns to produce outputs from a latent program representation. On the other hand








There are at least two primary hurdles in using evolutionary algorithms to synthesize programs.
{\em First}, it is non-trivial to design appropriate fitness functions.
Without a proper fitness function, an evolutionary algorithm may take a long time to (or never) converge. 
{\em Second}, evolutionary algorithms are often quick to find {\em close-enough} solutions but program synthesis requires exact solutions, which may take much longer to find. To address these 
challenges, we make two novel contributions. {\em First}, we use a neural network to automatically discover a suitable fitness function. The neural network determines which properties of candidate programs (i.e., \emph{genes} in evolutionary algorithm terminology) should be used as the fitness score.
In essence, we cast the design of a fitness function as a big data problem where a 
neural network learns to predict the quality of a gene by training on example programs.
{\em Second}, to move from approximate to precise program solutions, we occasionally check the local program space (i.e., {\em the neighborhood}) of some top scoring genes to search for an exact solution. Thus, we combine an evolutionary algorithm with occasional neighborhood
search to expedite the convergence process.

We have implemented these contributions in a framework, called {\em \scheme}, that 
synthesizes programs using an evolutionary algorithm. \scheme\ trains a neural network with
a set of programs (and their input-output examples) to predict various properties of those programs. We experimented with two different properties and compared 
their performance against Deepcoder's function probability based fitness score. Our results showed that \scheme\ performs better than Deepcoder's approach (e.g., $\mathbf{1.8\times}$ more synthesis rate).


%In Section ~\ref{sec-problem} we formalize the problem we are solving.  In Section ~\ref{sec-desc} we describe our solution to the problem.  Lessons learned are discussed in Section ~\ref{sec-lessons}.  Results are presented in Section ~\ref{sec-results} and comparisons made to related work in Section ~\ref{sec-rel}.  Finally, we draw conclusions in Section ~\ref{sec-conc}.

%For a given gene, the neural 
%network predicts properties such as how many functions might be common between this gene 
%and the solution or what is

%partly caused by the difficulty in finding appropriate fitness function. To overcome this %difficulty, this paper contributes with a novel approach 
%%to design fitness functions, 
%which is to use a neural network
%as a fitness function. Based on this idea, we propose an evolutionary framework to synthesize %program. The framework, called ESP, contains three novel contributions. 
%Among various machine learning
%bases synthesis techniques, Neural Program Synthesis
%techniques are particularly interesting because such
%techniques can produce actual programs by conditioning a neural network with input-output examples~\cite{}.

%Machine learning based program synthesis can be broadly categorized as Neural Program Induction techniques and Neural Program Synthesis technqiues. Neural Program Induction techniques~\cite{} strive to design a neural network that learns to produce outputs from a latent program representation. On the other hand


==> rel.tex <==
% !TEX root =  main.tex
Machine learning based program synthesis can be classified into two categories - neural
program synthesis and neural program induction. Deepcoder~\cite{deepcoder} is a promising 
approach for neural program synthesis. Neo extends Deepcoder to include information about
conflicting functions during the synthesis process~\cite{feng18}. Parisotto et al.~\cite{parisotto16} incrementally expands a partial program from continuous IO representations. Robustfill~\cite{robustfill} uses a modified RNN to encode 
variable-sized sets of I/O for synthesize string based programs.
Robinovich et al.~\cite{rabinovichSK17}
proposed to represent output as an abstract syntax tree which is then used by a decoder
to generate code. There is a growing amount of work in the domain of neural program
induction~\cite{neuralteuring, npi, npi2, cai17, fox18}, all proposing some neural
network design that can produce output directly from latent program representations.
Chen at el.~\cite{chen2018towards} propose a combination of non-differentiable machine, recursion and
reinforcement learning to generate a parsing program. There is a large body of work
that uses evolutionary algorithm for symbolic regression~\cite{Korns2011,Vladislavleva09,harper12}. However, the only work that comes
close to our work was proposed by Becker et al.~\cite{aip}.
%Becker et al.~\cite{aip} 
The work describes a program synthesis system built using an evolutionary algorithm on a low-level Turing complete language called \emph{BF}.  Their system required the user to provide 
%input/output examples, 
the target fitness score, and the rules to create the fitness function itself.
